Cost-Sensitive Self-Training for Optimizing Non-Decomposable Metrics

Self-training based semi-supervised learning algorithms have enabled the learning of highly accurate deep neural networks, using only a fraction of labeled data. However, the majority of work on self-training has focused on the objective of improving accuracy, whereas practical machine learning systems can have complex goals (e.g. maximizing the minimum of recall across classes, etc.) that are non-decomposable in nature. In this work, we introduce the Cost-Sensitive Self-Training (CSST) framework which generalizes the self-training-based methods for optimizing non-decomposable metrics. We prove that our framework can better optimize the desired non-decomposable metric utilizing unlabeled data, under similar data distribution assumptions made for the analysis of self-training. Using the proposed CSST framework, we obtain practical self-training methods (for both vision and NLP tasks) for optimizing different non-decomposable metrics using deep neural networks. Our results demonstrate that CSST achieves an improvement over the state-of-the-art in majority of the cases across datasets and objectives.

==> assets.tex <==
\section{Code, License, Assets and Computation Requirements}
\label{sec:code-licence-assets-comp-req}
\subsection{Code and Licenses of Assets}
In this work, we use the open source implementation of FixMatch~\cite{sohn2020fixmatch} \footnote{https://github.com/LeeDoYup/FixMatch-pytorch} in PyTorch, which is licensed under \ttt{MIT} License for educational purpose. Also for NLP experiments we make use of DistillBERT~\cite{sanh2019distilbert} pretrained model available in the HuggingFace~\cite{wolf2020transformers} library. The code to reproduce the main experiments results can be found at \href{https://github.com/val-iisc/CostSensitiveSelfTraining}{https://github.com/val-iisc/CostSensitiveSelfTraining}.

\subsection{Computational Requirements}
\begin{table}[htb]
\centering

\begin{tabular}{cccccccc} 
\toprule
    Method &  CIFAR-10 & CIFAR-100 & ImageNet-100 \\
     \hline
   \texttt{ERM}   &  \begin{tabular}{@{}c@{}}A5000 \\ 49m\end{tabular}  & \begin{tabular}{@{}c@{}}A5000 \\ 6h 47m\end{tabular} & \begin{tabular}{@{}c@{}} RTX3090 \\ 15h 8m\end{tabular} \\
   \texttt{LA}   &  \begin{tabular}{@{}c@{}}RTX3090 \\ 
39m\end{tabular}  & \begin{tabular}{@{}c@{}}A5000 \\ 6h 9m\end{tabular} & \begin{tabular}{@{}c@{}}A5000 \\ 15h 7m \end{tabular} \\
   \texttt{CSL}   &  \begin{tabular}{@{}c@{}}A5000 \\ 47m\end{tabular}  & \begin{tabular}{@{}c@{}}A5000 \\ 6h 40m\end{tabular} & \begin{tabular}{@{}c@{}}A5000 \\ 12h\end{tabular} \\
   \begin{tabular}{@{}c@{}}\texttt{CSST}(FixMatch)\\ w/o KL-Threshold\end{tabular} &  \begin{tabular}{@{}c@{}}4 X A5000 \\ 21h 0m\end{tabular}  & \begin{tabular}{@{}c@{}}4 X A100 \\ 2d 19h 16 m\end{tabular} & \begin{tabular}{@{}c@{}}4 X A5000 \\ 2d 13h 19m\end{tabular} \\
   \texttt{CSST}(FixMatch)    &  \begin{tabular}{@{}c@{}}4 X A5000 \\  21h 41m \end{tabular}  & \begin{tabular}{@{}c@{}}4 X A5000 \\2d 11h 52m \end{tabular} & \begin{tabular}{@{}c@{}}4 X A5000 \\ 2d 4m\end{tabular} \\
    \hline
\end{tabular}
\captionsetup{width=.68\textwidth}
\caption{Computational requirements and training time (d:days, h:hours, m:minutes) for  experiments relevant to vision datasets. As we can see some of the experiments on the larger datasets such as ImageNet requires long compute times.}
\label{tab:GPU-usage-vision}
\end{table}

\begin{table}[htb]
\centering
\begin{tabular}{cccccccc} 
\toprule
    Method &  IMDb($\rho=10$) & IMDb($\rho=100$) & DBpedia-14\\
     \hline
   \texttt{ERM}   &  \begin{tabular}{@{}c@{}}4 X A5000 \\ 25m \end{tabular}  & \begin{tabular}{@{}c@{} }4 X A5000 \\ 29m \end{tabular} & \begin{tabular}{@{}c@{}}4 X A5000 \\2h 44m\end{tabular} \\
   \texttt{UDA}   &  \begin{tabular}{@{}c@{}}4 X A5000 \\ 44m\end{tabular}  & \begin{tabular}{@{}c@{}}4 X A5000 \\ 32m\end{tabular} & \begin{tabular}{@{}c@{}}4 X A5000 \\ 10h 18m\end{tabular} \\
   \texttt{CSST}(UDA)    &  \begin{tabular}{@{}c@{}}4 X A5000 \\ 49m\end{tabular}  & \begin{tabular}{@{}c@{}}4 X A5000 \\ 35m\end{tabular} & \begin{tabular}{@{}c@{}}4 X A5000 \\ 13h 12m\end{tabular} \\
    \hline
\end{tabular}
\captionsetup{width=.68\textwidth}
\caption{Computational requirements and training time(d:days, h:hours, m:minutes)  for experiments done on NLP datasets. The DistilBERT model which we are using is pretrained on a language modeling task, hence it requires much less time for training in comparison to vision models which are trained from scratch.}
\label{tab:GPU-usage-nlp}
\end{table}

All experiments were done on a variety of GPUs, with primarily Nvidia A5000 (24GB) with occasional use of Nvidia A100 (80GB) and Nvidia RTX3090 (24GB). For finetuning DistilBERT and all experiments with ImageNet-100 dataset we used PyTorch data parallel over 4 A5000s. Training was done till no significant change in metrics was observed. The detailed list of computation used per experiment type and dataset have been tabulated in  Table \ref{tab:GPU-usage-vision} and Table \ref{tab:GPU-usage-nlp}.

==> experiment_details.tex <==

\section{Details of Experiments and Hyper-parameters}
\label{sec:appendix-details-of-experiments}
The experiment of $\max_F \min_i \text{recall}_i[f]$ and $\max_F \text{recall}[F] \text{ s.t. } \text{cov}_i[F] > \frac{0.95}{K}, \forall i \in [K]$  was performed on the long tailed version of CIFAR-10, IMDb($\rho=10,100$) and DBpedia-14 datasets. This was because the optimization of the aforementioned 2 objectives is stable for cases with low number of classes. Hence the objective of $\max_F \min(\text{recall}_{\mH}[F], \text{ recall}_{\mT}[F])$  and $\max_F \text{recall}[F] \text{ s.t. } \min_{\mH, \mT} \text{cov}_{\mH,\mT}[F] > \frac{0.95}{K}$ is a relatively easier objective for datasets with large number of classes, hence were the optimization objectives for CIFAR-100 and ImageNet-100 long tailed datasets. For all experiments for a given dataset, we used the same values for a given common hyperparameter. We ablated the threshold for our novel unlabeled sample selection criterion($\tau$) and the ratio of labeled and unlabeled samples, given fixed number of unlabeled samples($\mu$) and are available in Fig. \textcolor{red}{4b}.

\begin{table}[t]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{cccccccc} 
\toprule
    Parameter &  CIFAR-10 & CIFAR-100 & ImageNet-100 & \begin{tabular}{@{}c@{}}IMDb \\ ($\rho=10$)\end{tabular} & \begin{tabular}{@{}c@{}}IMDb \\ ($\rho=100$)\end{tabular}  &  DBpedia-14\\
     \hline
    $\tau$ &  0.05 & 0.05 & 0.05 & 0.1 & 0.1 & 0.1\\
    $\lambda_u$ & 1.0 & 1.0 & 1.0 & 0.1 & 0.1 & 0.1\\
    $\mu$ & 4.0 & 4.0 & 4.0 & 13.8 & 12.6 & 133\\
    $|B_s|$ & 64 & 64 & 64 & 32 & 32 & 32\\
    $|B_u|$ & 256 & 256 & 256 & 128 & 128 & 128\\
    lr & 3e-3 & 3e-3 & 0.1 & 1e-5 & 1e-5 & 1e-5\\
    $\omega$ & 0.25 & 0.25 & 0.1 & 0.5 & 0.5 & 0.5\\
    \begin{tabular}{@{}c@{}}SGD steps \\ before eval\end{tabular} &  32 & 100 & 500 & 50 & 50 & 100\\
    optimizer & SGD & SGD & SGD & AdamW & AdamW & AdamW \\
    KL-Thresh & 0.95 & 0.95 & 0.95 & 0.9 & 0.9 & 0.9 \\
    Weight Decay & 1e-4 & 1e-3 & 1e-4 & 1e-2 & 1e-2 & 1e-2\\
    $\rho$ &  100 & 10 & 10 & 10 & 100 & 100\\
    $\lambda_u$ &  1.0 & 1.0 & 1.0 & 0.1 & 0.1 & 0.1 \\
    $\mu$ &  4.0 & 4.0 & 4.0 & 11.0 & 11.0 & 11.0 \\
    Arch. &  WRN-28-2 & WRN-28-8 & ResNet50 & DistilBERT & DistilBERT & DistilBERT \\
    \hline
\end{tabular}
\end{adjustbox}
\caption{This table shows us the detailed hyper parameters used for \texttt{CSST}(FixMatch) for the long tailed datasets CIFAR-10, CIFAR-100, ImageNet-100 and \ttt{CSST}(UDA) on IMDb, DBpedia-14. All the datasets were converted to their respective long tailed versions based on the imbalance factor $\rho$, and a fraction of the samples were used along with their labels for supervision.}
\label{tab:hyperparams}
\end{table}
\vspace{-3mm}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
